Adaptive Influence Maximization in Social Networks: Why Commit when You can Adapt?

Most previous work on influence maximization in social networks is limited to the non-adaptive setting in which the marketer is supposed to select all of the seed users, to give free samples or discounts to, up front. A disadvantage of this setting is that the marketer is forced to select all the seeds based solely on a diffusion model. If some of the selected seeds do not perform well, there is no opportunity to course-correct. A more practical setting is the adaptive setting in which the marketer initially selects a batch of users and observes how well seeding those users leads to a diffusion of product adoptions. Based on this market feedback, she formulates a policy for choosing the remaining seeds. In this paper, we study adaptive offline strategies for two problems: (a) MAXSPREAD -- given a budget on number of seeds and a time horizon, maximize the spread of influence and (b) MINTSS -- given a time horizon and an expected number of target users to be influenced, minimize the number of seeds that will be required. In particular, we present theoretical bounds and empirical results for an adaptive strategy and quantify its practical benefit over the non-adaptive strategy. We evaluate adaptive and non-adaptive policies on three real data sets. We conclude that while benefit of going adaptive for the MAXSPREAD problem is modest, adaptive policies lead to significant savings for the MINTSS problem.

==> Future-Work.tex <==
\section{Future Work}
\label{sec:Future-Work}
We now outline some interesting directions for future work. For the case of bounded time horizon, we would like to explore Gaussian processes based Bayesian optimization techniques to find the optimal policy. Deriving explicit bounds for this scenario remains interesting future work. We would like to extend our framework to the linear threshold (LT) model and also for continuous time models. It will be interesting to derive theoretical results for the bandit setting of this problem or when we can obtain only partial information about the state of the network using some aggregate queries. We believe that with continuous time models and use of queries to infer the state of the network, adaptive influence maximization will be better able to model reality from a viral marketer's perspective. 
